Instrumental Variable Value Iteration for Causal Offline Reinforcement Learning

In offline reinforcement learning (RL) an optimal policy is learned solely from a priori collected observational data. However, in observational data, actions are often confounded by unobserved variables. Instrumental variables (IVs), in the context of RL, are the variables whose influence on the state variables is all mediated by the action. When a valid instrument is present, we can recover the confounded transition dynamics through observational data. We study a confounded Markov decision process where the transition dynamics admit an additive nonlinear functional form. Using IVs, we derive a conditional moment restriction through which we can identify transition dynamics based on observational data. We propose a provably efficient IV-aided Value Iteration (IVVI) algorithm based on a primal-dual reformulation of the conditional moment restriction. To our knowledge, this is the first provably efficient algorithm for instrument-aided offline RL.

==> b_4_2_npcase.tex <==

\subsection{Nonparametric Setting}
\label{sec:nonparacase}

In Assumptions~\ref{as:spec}~and~\ref{as:dualapprox} we make the simplifying assumption that both the true transition function $F^*$ and the image of the operator $\cT$ lies in a known finite-dimensional space. To extend our theory to the nonparametric case where $F^*:\cS\times\cA\to\R^{d_x}$ is H\"older continuous and functions of the form $\{\cT f\given f:\cS\times \cA\to\R \text{, bounded and continuous} \}$ are also H\"older continuous, we need to discuss two issues. 

The first is identification, that is, whether $F^*$ is the unique solution to conditional moment restriction in \cref{eq:thecondmoment}. Identification in nonparametric IV problems usually requires some form of completeness assumptions. For example, the bounded completeness condition is a relatively weak regularity assumption on the average visitation distribution $\bar d_{\pi_b}$. For two random variables $X$ and $Y$, $X$ is boundedly complete with respect to $Y$ if for all $Y$-a.s.~bounded function $f$, it holds that $\E[f(Y)\cond X]=0$ implies $f=0$ $Y$-a.s. Intuitively, it requires that the distribution of $Y$ exhibits a sufficient amount of variation when conditioning on different values of $X$. It is well known that there is a wide range of distributions that satisfy bounded completeness; see, for example, \citet{blundell2007semi}, \citet{d2011completeness}, \citet{Hu2017}, and \citet{Andrews2017}. 


The second issue is the error caused by the finite-dimensional approximation, which we address below. Let $f^*$ be one element of $F^*=[f^*_1,\dots, f^*_{d_x}]^\top$. If Assumption~\ref{as:spec} is violated, we define the primal approximation error as
$$
\eta_1 \defeq \| f^* - \Pi_\phi f^*\|_{\ltxa}.
$$
If Assumption~\ref{as:dualapprox} is violated, we define the dual error, which characterizes how well the dual function space $\Hpsi$ approximates functions of the form $\cT(f-f^*)$ for $f\in \Hphi$. We define 
$$
\eta_2 \defeq \sup_{} \{ \| \cT f - \Pi_\psi \cT f \|_{\ltz} : f\in \Hphi, \| f \|_{\ltxa} \leq 1 \}.
$$
Obviously, under Assumption~\ref{as:spec} we have $\eta_1=0$ and under Assumption~\ref{as:dualapprox} we have $\eta_2=0$.

The following result shows that, when Assumption~\ref{as:spec} and Assumption~\ref{as:dualapprox} are violated, the difference between $F^*$ and $W^\sad \phi$ linearly depends on the approximation errors $\eta_1$ and $\eta_2$. Recall that $f^*_i$ is the $i$-th element of $F^*=[f^*_1,\dots, f^*_{d_x}]^\top$, and $W^{\sad}_i $ is the $i$-th row of the estimand $\Wsad$ defined in \eqref{eq:estimatorw}. 

\begin{theorem}[Nonparametric setting] \label{lm:misspecification}
    Suppose that Assumptions~\ref{as:iiddata}--\ref{as:nonddualfeature} hold.
    Furthermore, assume that there is a constant $c>0$ such that 
    $\muIV \inv \cdot \|\cT(f^*_i - \Pi_\phi f^*_i )\|_{\ltz} \leq c\cdot \|f^*_i - \Pi_\phi f^*_i \|_{\ltxa}$.
    We define the operator $Q_{}\colon\ltxa \mapsto\Hphi$ as 
    \[
    Q_{} f = \argmin_{f'\in\Hphi} \| \Pi_{\psi}\cT(f'-f)\|_\ltz,
    \] 
    and let $\mu = \|(\Pi_\phi - Q_{})f^*_i \|_\ltxa$. Then it holds that
    \$
   \| f^*_i - W^{\sad}_i \cdot \phi\|_\ltxa \leq (1+2c) \cdot \eta_1 + \muIV \inv \cdot \mu \cdot \eta_2\,.
    \$
\end{theorem}
The existence of a constant $c$ in Theorem~\ref{lm:misspecification} is called the stability assumption; see \citet{blundell2007semi} and \citet{chen2018optimal} for a detailed discussion. Note that the dual approximation error $\eta_2$ is inflated by a factor of $\muIV\inv$. The estimation phase still produces an estimator that converges to $\Wsad$ at $O(1/T)$ rate. The only difference is that in the planning phase we are performing value iteration with a biased model.


==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{sec:intro}}.
  \item Did you describe the limitations of your work?
    \answerYes{See Remark~\ref{rm:globalivuc}}
  \item Did you discuss any potential negative societal impacts of your work?
  \answerNA{Not applicable. This is a theoretical work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  \answerNA{Not applicable. This is a theoretical work.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section \ref{sec:theory}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix \ref{app_proofs_of_theorems}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  \answerNA{Not applicable. This is a theoretical work.}
    \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{Not applicable. This is a theoretical work.}
    	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
      \answerNA{Not applicable. This is a theoretical work.}
      	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        \answerNA{Not applicable. This is a theoretical work.}
      \end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  \answerNA{Not applicable. This is a theoretical work.}
  \item Did you mention the license of the assets?
  \answerNA{Not applicable. This is a theoretical work.}
  \item Did you include any new assets either in the supplemental material or as a URL?
  \answerNA{Not applicable. This is a theoretical work.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  \answerNA{Not applicable. This is a theoretical work.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNA{Not applicable. This is a theoretical work.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
  \answerNA{Not applicable. This is a theoretical work.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA{Not applicable. This is a theoretical work.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{Not applicable. This is a theoretical work.}
\end{enumerate}

\end{enumerate}

